SEA: Sparse Linear Attention with Estimated Attention Mask

The transformer architecture has driven breakthroughs in recent years on tasks which require modeling pairwise relationships between sequential elements, as is the case in natural language understanding. However, long seqeuences pose a problem due to the quadratic complexity of the attention operation. Previous research has aimed to lower the complexity by sparsifying or linearly approximating the attention matrix. Yet, these approaches cannot straightforwardly distill knowledge from a teacher's attention matrix and often require complete retraining from scratch. Furthermore, previous sparse and linear approaches lose interpretability if they cannot produce full attention matrices. To address these challenges, we propose SEA: Sparse linear attention with an Estimated Attention mask. SEA estimates the attention matrix with linear complexity via kernel-based linear attention, then subsequently creates a sparse attention matrix with a top-k selection to perform a sparse attention operation. For language modeling tasks (Wikitext2), previous linear and sparse attention methods show roughly two-fold worse perplexity scores over the quadratic OPT-1.3B baseline, while SEA achieves better perplexity than OPT-1.3B, using roughly half the memory of OPT-1.3B, providing interpretable attention matrix. We believe that our work will have a large practical impact, as it opens the possibility of running large transformers on resource-limited devices with less memory.

==> tables/ablation_topk.tex <==
\begin{table}[h]
\caption{Ablation study on grouped top-k modes: per-query, per-head, and per-batch. The model is evaluated on Glue-MNLI with BERT-base ($K=128$), until 5 epochs.}
\label{table.ablation.topk}
\begin{center}
\begin{tabular}{l|ccc}
\toprule
         Top-$k$ Grouping Method   & $k=7$ & $k=13$ & $k=25$ \\
\midrule
\textit{per-query} & 77.68 & 81.45 & 83.55 \\
\textit{per-head} & 79.03 & 82.71 & 83.71 \\ 
\textit{per-batch} & 80.03 & 82.94 & 84.14 \\
\rowcolor{teagreen}\textit{\textbf{causal per-batch}} & \textbf{80.55} & \textbf{83.49} & \textbf{84.19} \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

